Advancing Transformer Architecture in Long-Context Large Language Models: A Comprehensive Survey

Transformer-based Large Language Models (LLMs) have been applied in diverse areas such as knowledge bases, human interfaces, and dynamic agents, and marking a stride towards achieving Artificial General Intelligence (AGI). However, current LLMs are predominantly pretrained on short text snippets, which compromises their effectiveness in processing the long-context prompts that are frequently encountered in practical scenarios. This article offers a comprehensive survey of the recent advancement in Transformer-based LLM architectures aimed at enhancing the long-context capabilities of LLMs throughout the entire model lifecycle, from pre-training through to inference. We first delineate and analyze the problems of handling long-context input and output with the current Transformer-based models. We then provide a taxonomy and the landscape of upgrades on Transformer architecture to solve these problems. Afterwards, we provide an investigation on wildly used evaluation necessities tailored for long-context LLMs, including datasets, metrics, and baseline models, as well as optimization toolkits such as libraries, frameworks, and compilers to boost the efficacy of LLMs across different stages in runtime. Finally, we discuss the challenges and potential avenues for future research. A curated repository of relevant literature, continuously updated, is available at https://github.com/Strivin0311/long-llms-learning.

==> chapters/acknowledgement.tex <==
\section*{Acknowledgement}

We would like to express our gratitude to Hao Gao for their helpful discussions and feedback during the early stages of this paper. We also extend our appreciation to our Baidu colleagues, including Hao Chen, Linyun Liu, PengHao Zhao, and others, for their contributions and insights in the initial research phases.

Additionally, we acknowledge the generous support from the Baidu AI Cloud Group (ACG). We are especially thankful to Dou Shen, the Executive Vice President and Head of ACG, for the great idea and gracious invitation to the first session of Baidu ACG Summer Camp. This opportunity has been instrumental in shaping our research and providing valuable experiences.

==> chapters/reference.tex <==
\bibliographystyle{plain}
% \bibliographystyle{plainurl}
% \bibliographystyle{alphabetic}

\bibliography{ref-arxiv-v1}
    
% \bibliography
% {
%     refs/background, 
%     refs/base, 
%     refs/benchmarks, 
%     refs/context_processing, 
%     refs/efficient_attention, 
%     refs/extrapolative_pe, 
%     refs/llms, 
%     refs/long_term_memory, 
%     refs/survey, 
%     refs/miscellaneous,
%     refs/platform,
% }
